DeepRecSys: A System for Optimizing End-To-End At-scale Neural Recommendation Inference

Neural personalized recommendation is the corner-stone of a wide collection of cloud services and products, constituting significant compute demand of the cloud infrastructure. Thus, improving the execution efficiency of neural recommendation directly translates into infrastructure capacity saving. In this paper, we devise a novel end-to-end modeling infrastructure, DeepRecInfra, that adopts an algorithm and system co-design methodology to custom-design systems for recommendation use cases. Leveraging the insights from the recommendation characterization, a new dynamic scheduler, DeepRecSched, is proposed to maximize latency-bounded throughput by taking into account characteristics of inference query size and arrival patterns, recommendation model architectures, and underlying hardware systems. By doing so, system throughput is doubled across the eight industry-representative recommendation models. Finally, design, deployment, and evaluation in at-scale production datacenter shows over 30% latency reduction across a wide variety of recommendation models running on hundreds of machines.

==> casestudy.tex <==

\section{Case Study I: Future datacenter infrastructure}

Application specific accelerators can be used to accelerate a subset of models.
As an example we study the performance benefits of GPUs.
GPUs work well for compute intensive models but not models dominated by irregular memory accesses.

Takeaway: Accelerators are good for speeding up a subset of models however, if there is a large tail in model architecture (shown in HPCA submission) then general purpose CPU platforms offer a good alternative.

\section{Case Study II: Deploying large models}

In addition to exploiting the tail-latency benefits of judiciously balancing task, model, and data-level parallelism for infrastructure efficiency (i.e., maximizing QPS), the additional slack can be used to deploy larger models.
Generally, it is shown that model accuracy scales with the size of deep learning models ~\cite{}.
Typically we find that the personalized recommendation models are limited by the strict tail-latency targets set by SLAs.
However, deploying larger models can provide higher accuracy translating to improved user experience through better recommendations.
As a result, the optimizations proposed here can be leveraged to deploy larger models.
This section uses the flexible and extensible framework to evaluate the bound of the new model capacity.

For the purposes of this case study we focus on three of the six state-of-the-art personalized recommendation models. Study bounds that are unique to personalized recommendation.

\textbf{DLRM} How many more embedding table lookups can we run?

\textbf{Multi-task wide and deep} How many more tasks can we support?

\textbf{Deep interest evolution} Length of user-behavior sequence we can run?

We leave it to future work to demonstrate the end-to-end accuracy benefits of these models expansions.



==> characterization.tex <==
\section{Design space exploration}
% Characterization of design space sweep
At-scale execution of personalized recommendation models requires achieving high-throughput while meeting strict tail latency targets set by service level argreements (SLAs).
These SLAs vary based on the application in which personalized recommendation models are used.
For instance, low-latency search as requirements on the order of tens of milliseconds~\cite{wnd} while social media platforms have requirements on the order of hundreds of milliseconds.
In addition to application diversity, the diversity in personalized recommendation models introduces different optimization opportunities.
In particular, for at-scale deployment we can balance different parallelization opportunities including: task, model, and data-level parallelism.
This section illsutrates the optimization design-space for parallelization opportunities for the differnt model architectures.

\subsection{Task versus model-level parallelism}
Show task vs. model level parallelism for 2 different models.

\subsection{Data level parallelism}
Show opportunity for data-level parallelism for 2 different model architectures.

\subsection{Overview}
Show pareto optimal configuration for the different models.
Perhaps annotate the pareto-optimal points for all configurations (Scatter plot).

